Continuously bounds-preserving discontinuous Galerkin methods for hyperbolic conservation laws

For finite element approximations of transport phenomena, it is often necessary to apply a form of limiting to ensure that the discrete solution remains well-behaved and satisfies physical constraints. However, these limiting procedures are typically performed at discrete nodal locations, which is not sufficient to ensure the robustness of the scheme when the solution must be evaluated at arbitrary locations (e.g., for adaptive mesh refinement, remapping in arbitrary Lagrangian--Eulerian solvers, overset meshes, etc.). In this work, a novel limiting approach for discontinuous Galerkin methods is presented which ensures that the solution is continuously bounds-preserving (i.e., across the entire solution polynomial) for any arbitrary choice of basis, approximation order, and mesh element type. Through a modified formulation for the constraint functionals, the proposed approach requires only the solution of a single spatial scalar minimization problem per element for which a highly efficient numerical optimization procedure is presented. The efficacy of this approach is shown in numerical experiments by enforcing continuous constraints in high-order unstructured discontinuous Galerkin discretizations of hyperbolic conservation laws, ranging from scalar transport with maximum principle preserving constraints to compressible gas dynamics with positivity-preserving constraints.

==> scratch.tex <==
\section{Bounding concave functionals}\label{app:bounds}
Let the solution be represented through a monomial basis as per \cref{eq:modal} and \cref{eq:monomial}, e.g., for a two-dimensional scalar solution of order $p$ on a quadrilateral element, 
\begin{equation}
    u(\hat{\mathbf{x}}) = \sum_{i=0}^{p}\sum_{j=0}^{p} u_{ij} \hat{x}^i \hat{y}^j.
\end{equation}
We assume the reference element $\hat{\Omega}$ is appropriately normalized such that $-1 \leq \hat{x}, \hat{y} \leq 1$. We seek an appropriate upper/lower bound on the solution on some convex subdomain $\mathcal D = [\hat{x}_1, \hat{x}_2] \times [\hat{y}_1, \hat{y}_2]$ where $\hat{x}_2 > \hat{x}_1$, $\hat{y}_2 > \hat{y}_1$ and $\mathcal D \subset \hat{\Omega}$ (e.g., some tessellation of the reference element such as the subcells created from a set of sampled nodes). The local monotonicity of monomials can be exploited to show that 
\begin{equation}
    \underset{a \leq z \leq b}{\max} z^p = \max ( a^p, b^p),
\end{equation}
and 
\begin{equation}
    \underset{a \leq z \leq b}{\min} z^p = \begin{cases}
        \min ( a^p, 0, b^p), \quad \text{if $a < 0$ and $b > 0$},\\
        \min ( a^p, b^p), \quad \quad \text{else}.
    \end{cases} 
\end{equation}
Therefore, we can bound the minimum and maximum of the $ij$-th basis function of $u(\hat{\mathbf{x}})$ over the subdomain $\mathcal D$ by taking the discrete extrema of the permutations, i.e.,
\begin{equation}
    u^{\min}_{ij} = \min \left(u_{ij} \hat{x}_{\min} \hat{y}_{\min}, 
    u_{ij} \hat{x}_{\min} \hat{y}_{\max},
    u_{ij} \hat{x}_{\max} \hat{y}_{\min},
    u_{ij} \hat{x}_{\max} \hat{y}_{\max}\right)
\end{equation}
and 
\begin{equation}
    u^{\max}_{ij} = \max \left(u_{ij} \hat{x}_{\min} \hat{y}_{\min}, 
        u_{ij} \hat{x}_{\min} \hat{y}_{\max},
        u_{ij} \hat{x}_{\max} \hat{y}_{\min},
        u_{ij} \hat{x}_{\max} \hat{y}_{\max}\right).
\end{equation}
These can then be combined to yield a lower and upper bound for $u(\hat{\mathbf{x}})$ over the subdomain $\mathcal D$ as
\begin{equation}
    u^{\min} = \sum_{i=0}^{p}\sum_{j=0}^{p} u_{ij}^{\min} \quad  \text{and} \quad u^{\max} = \sum_{i=0}^{p}\sum_{j=0}^{p} u_{ij}^{\max}.
\end{equation}
For general nonlinear strictly concave or non-convex constraint functionals of scalar-valued solutions, this is sufficient to bound the constraint functional as
\begin{equation}
    g^{\min} = \min \left( g(u^{\min}),  g(u^{\max})\right).
\end{equation}
To extend this to functionals of vector-valued solutions, the bounds for the extrema of each component can be computed and the concavity (or, more strictly speaking, the non-convexity) of $g$ can be exploited to compute $g^{\min}$ as the discrete minima of the permutations as above, e.g., for a two-component system $\mathbf{u} = [u_1, u_2]^T$,
\begin{equation}
    g^{\min} = \min \left( g(u^{\min}_1,u^{\min}_2),  g(u^{\min}_1,u^{\max}_2),
    g(u^{\max}_1,u^{\min}_2),
    g(u^{\max}_1,u^{\max}_2)\right).
\end{equation}
